Algorithmic Challenges in Ensuring Fairness at the Time of Decision

Algorithmic decision-making in societal contexts, such as retail pricing, loan administration, recommendations on online platforms, etc., can be framed as stochastic optimization under bandit feedback, which typically requires experimentation with different decisions for the sake of learning. Such experimentation often results in perceptions of unfairness among people impacted by these decisions; for instance, there have been several recent lawsuits accusing companies that deploy algorithmic pricing practices of price gouging. Motivated by the changing legal landscape surrounding algorithmic decision-making, we introduce the well-studied fairness notion of envy-freeness within the context of stochastic convex optimization. Our notion requires that upon receiving decisions in the present time, groups do not envy the decisions received by any of the other groups, both in the present as well as the past. This results in a novel trajectory-constrained stochastic optimization problem that renders existing techniques inapplicable. The main technical contribution of this work is to show problem settings where there is no gap in achievable regret (up to logarithmic factors) when envy-freeness is imposed. In particular, in our main result, we develop a near-optimal envy-free algorithm that achieves $\tilde{O}(\sqrt{T})$ regret for smooth convex functions that satisfy the PL inequality. This algorithm has a coordinate-descent structure, in which we carefully leverage gradient information to ensure monotonic sampling along each dimension, while avoiding overshooting the constrained optimum with high probability. This latter aspect critically uses smoothness and the structure of the envy-freeness constraints, while the PL inequality allows for sufficient progress towards the optimal solution. We discuss several open questions that arise from this analysis, which may be of independent interest.

==> figures/algorithm2.tex <==

\begin{algorithm}[tb]
\footnotesize
\DontPrintSemicolon
\SetKwInOut{Input}{input}
\Input{convexity parameters $\alpha$, $\beta$, time horizon $T$, feasible set $\mathcal{X}=[x_{\min},x_{\max}]$, initial lag size $\delta_1$, stopping parameter $\gamma > 1$, $q \in (0,1)$, noise sub-Gaussian norm bound $E_{\max}$, Hoeffding constant $C$} 
$\delta_i \leftarrow q^{i-1} \delta_1$ for $i \geq 2$, $\xi \leftarrow 1 - q$, $n(d) = \frac{64 E_{\max}^2 \log \frac{2}{p}}{C\alpha^2 d^4}$ for any $d$, $x_1 \leftarrow x_{\min} + \delta_1$, $t \leftarrow 1$, $i \leftarrow 0$ \;
\Repeat{$T$ samples have been taken}{
    $i \leftarrow i - 1$ \;
    \Repeat{$-\frac{1}{\beta} g_t^{(i)} \geq (2+\gamma) \delta_i$}{
        $i \leftarrow i + 1$ \;
        $\overline{f}(x_t - \delta_i) \leftarrow$ average of $n(\xi \delta_i)$ samples at $x_t - \delta_i$ \tcp*[f]{estimate $f(x_t-\delta_i)$} \;
        $\overline{f}(x_t - \delta_{i+1}) \leftarrow$ average of $n(\xi \delta_i)$ samples at $x_t - \delta_{i+1}$ \tcp*[f]{estimate $f(x_t-\delta_{i+1})$}\;
        $g_t^{(i)} \leftarrow \frac{\overline{f}(x_t - \delta_{i+1}) - \overline{f}(x_t - \delta_{i}) + \alpha \xi^2 \delta_i^2/4}{\xi \delta_i}$ \tcp*[f]{compute the approximate secant}\;
    }
    $\overline{f}(x_t) \leftarrow$ average of $n(\delta_i)$ samples at $x_t$ \tcp*[f]{estimate $f(x_t)$} \;
    $\tilde{\tilde{\nabla}}_t \leftarrow \frac{\overline{f}(x_t) - \overline{f}(x_t - \delta_{i}) + \alpha \delta_i^2/4}{\delta_i}$ \tcp*[f]{compute the approximate secant} \;
    Compute $x_{t+1} \leftarrow x_t - \frac{1}{\beta} \tilde{\tilde{\nabla}}_t - \delta_i$\;
    \If{$x_{t+1} > x_{\max}$}{
        Set $x_s \leftarrow x_{\max}$ for all $t+1 \leq s \leq T$
    }
    $t \leftarrow t + 1$ \;
}
\caption{Adaptive Lagged Gradient Descent ({\sc Ada-Lgd})}
\label{alg:continual-lgd}
\end{algorithm}


==> figures/nd-algorithm.tex <==
\begin{algorithm}[h]
\footnotesize
\DontPrintSemicolon
\SetKwInOut{Input}{input}
\Input{Number of groups $N$, \js{sub-Gaussian norm bound $E_{\max}$, $n(d) = \frac{64 E_{\max}^2 \log \frac{2}{p}}{C\alpha^2 d^4}$,} smoothness parameter $\beta$ and strong convexity parameter $\alpha$ of $f(x_1,\ldots,x_N) = \sum_{i=1}^N f_i(x_i)$, time horizon $T$, non-negative FTP slacks $s$, \js{$x_{\min}$,} $\gamma$, lag size $\delta$} 
Initialize queue $Q_i \leftarrow \emptyset$ for $i \in [N]$ \tcp*[f]{will contain points to query} \; %\sge{is this each group or as you vary the partition is it for each member of the partition?} \js{When groups are combined, the cluster is assigned a "representative group" which is just the minimum index group (see line 11). The points to query are then added to the queue for that representative group.}}  \;
Initialize the partition $\Pi = \big\{ \{1\},\ldots,\{N\} \big\}$ of groups, and set $\textup{active}_A = \textup{Yes}$ and $g_A = -\infty$ for each $A \in \Pi$ \;
For any $A \subseteq [N]$, define $f_A(x) = \sum_{i \in A} f_i(x)$; initialize $A = \{1\}$ \;
Add \js{$x_{\min}$, $x_{\min}+\delta$} to $Q_i$ for $i \in [N]$ \;
% Sample $f_1$ and $f_2$ for $n(\xi \delta)$ times at $x_1-\delta$ and $x_2-\delta$, respectively \;
% $i \leftarrow 1$ \tcp*[f]{segment to be moved (either 1 or 2)} \;
\While{fewer than $T$ samples have been taken}{
    \If{$\textup{active}_B = \textup{No}$ for each cluster $B \in \Pi$ \js{(i.e., no clusters can move)}}{
        \uIf{each cluster is constrained by some other cluster}{
            Find clusters $C,D$ which are locked in place with respect to each other \js{(see Claim~\ref{claim:existence-of-low-gradient})}
        }
        \Else{
            Find clusters $C \ne D \in \Pi$ such that $C$ is at a tight constraint imposed by some group in $D$, and $D$ has met the small gradient condition \js{(see Claim~\ref{claim:existence-of-low-gradient})} \;%\sg{why should this happen?}\js{We know that they can't all be at a low gradient, by line 26. So, there must be at least one cluster at a tight constraint. Look at a cluster that constrains the first. If it's at a low gradient, we're done. Otherwise, look at a cluster that constrains the second. If it's at a low gradient, we're done. Otherwise, keep going until you've reached the last. It must be at a low gradient, since it cannot be constrained by any of the previous ones.}\;
        }
        Update $\Pi \leftarrow \Pi \cup \{C \cup D\} \setminus \{C,D\}$ \;
        Let $A = C \cup D$, and set $g_{A} = -\infty$ and $\textup{active}_A = \textup{Yes}$\;
        Let $i = \min A$, and add $x_i, x_i+\delta$ to $Q_i$ \tcp*[f]{\js{add points to the representative group's queue}}
    }
    Let $i = \min A$ \tcp*[f]{choose a representative group} \;
    $\mathcal{X}_A = [x_i, x_i + d(A;x)]$ \tcp*[f]{current feasible points for cluster $A$}\;
    \If{$Q_i$ contains any elements in $\mathcal{X}_A$}{
        Let $x_i \leftarrow \min Q_i$, remove $x_i$ from $Q_i$, and update $x_j$ (for $j \in A \setminus \{i\}$) accordingly \js{(i.e., letting $d = \min Q_i - x_i$, we set $x_j \leftarrow x_j + d$ for all $j \in A$)}\; 
        Update $\textup{active}_B$ for $B \in \Pi$ as necessary (formerly tight clusters \js{may} now be active; \js{in particular, if $B$ is at a tight constraint imposed by some group in $A$ and $B$ is not at any tight constraints imposed by any group in any other cluster, then $B$ will no longer be at a tight constraint}) \;%\sge{make this more precise? the tight clusters with the tight constraint in A?} \;
        Sample $n(\delta)$ times at \js{$x_j$ for $j \in A$} \;
        \If{$x_i$ is a non-lagged iterate for cluster $A$}{
            Update the gradients $g^{(i)}$ for $i \in A$  and set $g_A = \sum_{i \in A} g^{(i)}$ \;
            \uIf{$-\frac{1}{\beta} g_A \geq (1+\gamma)\delta$}{
                Add $x_i - 2\delta - \frac{1}{\beta}g_A$ and $x_i - \delta - \frac{1}{\beta}g_A$ to $Q_i$ \;
            }
            \Else{
                Set $\textup{active}_A = \textup{No}$
            }
        }
    }
    \If{$Q_i$ contains no elements in $\mathcal{X}_A$}{
        Set $x_i = \max \mathcal{X}_A$ and update $x_j$ (for $j \in A$) accordingly \;
        Set $\textup{active}_A = \textup{No}$ and update $\textup{active}_B$ for $B \in \Pi$ (formerly tight clusters may now be active) 
    }
    
    
    \If{$-\frac{1}{\beta}g_B < (1+\gamma) \delta$ for every cluster $B \in \Pi$}{
        Exit the while loop and remain at point $x$ for the remaining iterations
    }
    $A \leftarrow \varphi(A;\Pi)$ \tcp*[f]{move to the next group}\;
}

% \While{fewer than $T$ samples have been taken}{
%     {\bf Combined phase:}\\
%     Run \textsc{Adaptive Lgd} on the combined function ($h(x)=f_1(x)+f_2(x+s(2,1))$ if Segment 2 is at the facet, $h(x)=f_1(x+s(1,2))+f_2(x)$ otherwise), using the previously sampled lagged points (with lags $\delta^{(-i)}$ and $q\delta^{(-i)}$), smoothness parameter $2\beta$, and strong convexity parameter $2\alpha$.
% }

\caption{Cycle-then-Combine Lagged Gradient Descent ({\sc C$^2$-Lgd})}%FTP} 
\label{alg:multi-segment}
\end{algorithm}

==> figures/shorter-algorithm-2group.tex <==
\begin{algorithm}[!t]
\scriptsize
\DontPrintSemicolon
\SetKwInOut{Input}{input}
\Input{initial point $(x_1,x_2)$, smoothness $\beta \geq 1$ of the objective function $f(x_1,x_2) = f_1(x_1) + f_2(x_2)$, horizon $T$, slacks $s(1,2), s(2,1)$, $x_{\min}$, $\gamma$, $q \in (0,1)$, $\xi = 1-q$, %\sge{\sout{$D(d) = (2+\gamma) \frac{\beta}{\alpha} \cdot \frac{d}{q}$, $H(d) = (\frac{\beta}{\alpha}-1)D(d) + \frac{\beta d}{\alpha}$}},
initial lag $\delta = \delta^{(1)} = \delta^{(2)}$,  %sub-Gaussian norm bound $E_{\max}$, 
$\textsc{Grad}(x,y)= \frac{\overline{f}(y) - \overline{f}(x)}{y-x}$, where $\overline{f}$ is the average of $n(y-x)$ function value samples, where $n(d) = \frac{2 E_{\max}^2 \log \frac{2}{p}}{d^4}$, and gradient adjustments $\varepsilon_1(x) = (1+\beta)x$ and $\varepsilon_2(x) = x$}%, where $E_{\max}$ is a bound on the noise, and $C$ is the Hoeffding constant.}
Initialize queues to maintain tuples of (sampling point, number of samples, and the type of sampling point $(S)$):
$Q_1 = Q_2 = \{\big(x_{\min}, n(\xi \delta), S=1\big)$, $\big(x_{\min}+\xi\delta, n(\xi q\delta), S=2\big)$, $\big(x_{\min}+\delta, n(\delta),S=0\big)$\}\; 
\tcp*{$S=k>0$ represents the $k$th lagged point, $S=0$ represents a non-lagged point, and $S\in\{-1,-2\}$ represents the two feasibility iterates.}
% Initialize $x_1 = x_2 = x_{\min}$\;
\textbf{Coordinate Descent Phase:}\; 
\While{fewer than $T$ samples have been taken}{

    $\mathcal{X}_i = [x_i, x_{-i}+s(i,-i)]$ for $i=1,2$ \tcp*[f]{current feasible points for Group $i= 1,2$}\;
    \textbf{if} $\exists j: Q_j \cap \mathcal{X}_j \neq \emptyset$ \textbf{then} Set $i \in \{j ~|~ Q_j \cap \mathcal{X}_j \ne \emptyset\}$; %\tcp*[f]{we overload $Q_j \cap \mathcal{X}_j$ notation to mean iterates in $Q_j$ that lie in $\mathcal{X}_j$}\;
    {\bf else} go to {\bf Combined Phase} (line 11)\;
    set \texttt{switch} = False\;
    \While{$Q_i \cap \mathcal{X}_i \ne\emptyset$}{ 
        %SWITCH = false; 
        {\bf Sample:} Let $(x_i, n_x, S_i)$ be the lowest point to sample in $Q_i \cap \mathcal{X}_i$ by first coordinate (with ties broken arbitrarily) and obtain $n_x$ %$X^{(i)}_{x_i} \in \mathbb{R}^{n_x}$ by 
        samples of $f_i(x_i)$; Update $Q_i \leftarrow Q_i \setminus (x_i, n_x, S_i)$\;
        \textbf{Gradient checks based on type ($S_i$) of $x_i$}:\;
        \begin{enumerate}
            %\item \textbf{if} $x_i$ is the first of the lagged iterates, \textbf{then} do nothing \;
            \item[(a)] \textbf{if} $x_i$ is a $j$th lagged point (i.e., $S_i=j$) and $j>1$ \textbf{then} \;
                \hspace{1.3cm} \textbf{if} $-\textsc{Grad}((j-1)\text{st}~\mbox{lagged point},x_i) - \varepsilon_1(\delta^{(i)}) \leq \gamma \delta^{(i)}$:\;
                \hspace{2cm} Plan to sample next lagged point: $Q_i \leftarrow Q_i \cup$ $\{\big(x_i+\xi q \delta^{(i)}, n(\xi q \delta^{(i)}), S=j+1\big)\}$ \;
                \hspace{2cm} $\delta^{(i)} \leftarrow q\delta^{(i)}$ and adjust the sample size for the next non-lagged iterate in $Q_i$ to $n(\delta^{(i)})$\; 
            \item[(b)] \textbf{if} $x_i$ is a non-lagged point (i.e., $S_i = 0$) \textbf{then} \;
                \hspace{1.3cm} Let $g = \textsc{Grad}(x_i-\delta^{(i)},x_i) + \varepsilon_2(\delta^{(i)})$\;
                \hspace{1.3cm} \textbf{if} $-\frac{1}{\beta} g < T^{-1/4}$  \textbf{then} set $Q_i \leftarrow \emptyset$ (never move group $i$ in coordinate descent again)\;
                \hspace{1.3cm} \textbf{else} 
                populate queue with the next non-lagged and lagged points:\; 
                \hspace{2cm} Let $y = x_i - \delta^{(i)} - \frac{1}{\beta} g$, and\;
                \hspace{2cm} $Q_i \leftarrow Q_i \cup \{(y-\delta^{(i)},n(\xi \delta^{(i)}), S=1), ~(y-q\delta^{(i)},n(\xi q \delta^{(i)}), S=2)$, $(y,n(\delta^{(i)}), S=0)$\}\;
                \hspace{1.3cm} \textbf{if} lagged size has dropped enough so that $\delta^{(i)} < \delta^{(-i)}$, then switch group: \texttt{switch} = True\;
            \item[(c)] \textbf{if} $x_i$ is the second feasibility iterate (i.e., $S_i = -2$) \textbf{then} \;
                \hspace{1.3cm} Let $g = \textsc{Grad}(\mbox{previous feasibility iterate},x_i)$\;
                \hspace{1.3cm} \textbf{if} $-\frac{1}{\beta} g \geq  \Big(\frac{(2+\gamma)\beta}{q \alpha}+1\Big) \delta^{(-i)}$ \textbf{then} \;
                \hspace{2cm} set $Q_1,Q_2 \leftarrow \emptyset$ (i.e., enter the combined phase) \;
                \hspace{1.3cm} \textbf{else if} $Q_{-i} = \emptyset$ \textbf{then} sample at $(x_1,x_2)$ for the remaining time until $T$\;
        \end{enumerate} 
        {\bf Add feasibility iterates:} \textbf{if} %we are about to switch groups and group $i$ is at a lower lag size (i.e., 
        (\texttt{switch} = True or $Q_i \cap \mathcal{X}_i = \emptyset$) AND $\delta^{(i)} < \delta^{(-i)}$  %\js{SWITCH=true or there are no further points in $Q_i \cap X_i$, AND group $i$ is at a lower lag size, i.e., } $Q_i \cap \mathcal{X}_i = \emptyset$ \js{\textbf{and}} $\delta^{(i)} < \delta^{(-i)}$ 
        \textbf{then}\; 
        \hspace{1.3cm}set $\mathcal{X}_{-i} \leftarrow [x_{-i}, x_i + s(-i,i)]$\;
        \hspace{1.3cm}$Q_{-i} \leftarrow Q_{-i} \cup \{\big(\max \mathcal{X}_{-i} - \delta^{(i)}, n(\xi \delta^{(i)}), S=-1\big), \big(\max \mathcal{X}_{-i} - q\delta^{(i)}, n(\xi q\delta^{(i)}), S = -2\big)\}$\;
        \hspace{1.3cm}switch groups: $i \leftarrow -i$ 
        }
    }
{\bf Combined phase:}\\
\While{fewer than $T$ samples have been taken}{
    Run \textsc{Ada-Lgd} with previously sampled lagged points (with lags $\delta^{(-i)}$ and $q\delta^{(-i)}$) on function $\psi$: \\
        \hspace{1cm}\textbf{if} Group 2 is tight, set $\psi(x)=f_1(x)+f_2(x+s(2,1))$; \textbf{else} set $\psi(x)=f_1(x)+f_2(x-s(1,2))$
}
\caption{Switch-then-Combine Adaptive Lagged Gradient Descent ({\sc SCAda-Lgd})}%Noisy Bandit 2-Group Asymmetric FTP} 
\label{alg:noisy-2segment-asymmetric-simplified-v2}
\end{algorithm}
